Personalized Emotion Detection from Floor Vibrations Induced by Footsteps

Emotion recognition is critical for various applications such as early detection of mental health disorders and emotion based smart home systems. Previous studies used various sensing methods for emotion recognition, such as wearable sensors, cameras, and microphones. However, these methods have limitations in long term domestic, including intrusiveness and privacy concerns. To overcome these limitations, this paper introduces a nonintrusive and privacy friendly personalized emotion recognition system, EmotionVibe, which leverages footstep induced floor vibrations for emotion recognition. The main idea of EmotionVibe is that individuals' emotional states influence their gait patterns, subsequently affecting the floor vibrations induced by their footsteps. However, there are two main research challenges: 1) the complex and indirect relationship between human emotions and footstep induced floor vibrations and 2) the large between person variations within the relationship between emotions and gait patterns. To address these challenges, we first empirically characterize this complex relationship and develop an emotion sensitive feature set including gait related and vibration related features from footstep induced floor vibrations. Furthermore, we personalize the emotion recognition system for each user by calculating gait similarities between the target person (i.e., the person whose emotions we aim to recognize) and those in the training dataset and assigning greater weights to training people with similar gait patterns in the loss function. We evaluated our system in a real-world walking experiment with 20 participants, summing up to 37,001 footstep samples. EmotionVibe achieved the mean absolute error (MAE) of 1.11 and 1.07 for valence and arousal score estimations, respectively, reflecting 19.0% and 25.7% error reduction compared to the baseline method.

==> Sections/not_used/03Method.tex <==
\section{EmotionVibe: Emotion Recognition System Using Footstep-Induced Floor Vibration Signals}
The main objective of EmotionVibe is to recognize people's emotions, specifically estimating their valence and arousal scores, based on the floor vibrations induced by their footsteps. EmotionVibe mainly consists of three parts as shown in Figure~\ref{fig:system}: (1) Vibration-to-feature processing, (2) General emotion recognition development, and (3) Personalized emotion recognition development.
% Initially, we capture the footstep-induced floor vibration signals using vibration sensors attached to the floor. Subsequently, these signals undergo preprocessing including segmenting each footstep signal and calibrating the clipping effect for feature extraction and further process. Following this, emotion-sensitive features are extracted from the preprocessed signals. The general emotion recognition model is trained using the extracted features from the individuals' data in the training set. Each individual's data in the training set is given equal weight in the modeling process. To ensure the model fits within a limited dataset size, we simplify its complexity through an iterative pruning process that gradually eliminates the least significant parameters. Subsequently, we compare the gait similarity between the target individual and those in the training set by analyzing floor vibrations, using similarity indices to represent each individual's gait similarity with the target person. Individuals with more similar gait patterns will have higher similarity indices. Finally, the personalized emotion recognition model is constructed by assigning the similarity indices as weights for the training data, thereby enabling the development of a person-specific emotion recognition model for the target person.

% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=0.8\linewidth]{Figs_v2/system_overview_v1.pdf}
%   \caption{EmotionVibe System Overview.}
%   \label{fig:system}
% \end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{Figs/system_overview_v12.pdf}
  \caption{EmotionVibe System Overview.} 
  \label{fig:system}
\end{figure}
% The system starts with collecting footstep-induced floor vibration signals, followed by preprocessing to enhance signal quality for feature extraction. Subsequently, emotion-sensitive features are extracted. A general emotion recognition model is developed using training data (from $P_1$, $P_2$, ..., $P_n$) and then iteratively pruned to simplify the model's complexity by removing the least important parameters. This general model serves as the baseline. In addition, the general model's hidden layers, which map floor vibrations to gait patterns, enable gait similarity comparisons between the target person's ($P_T$) data and the training dataset. These similarity indices are assigned to the samples as weights for personalized emotion recognition modeling. The personalized emotion recognition model estimates emotion scores (valence and arousal) based on the floor vibration signals.
\subsection{Vibration-to-Feature Processing}
In this section, we first describe the methods used to collect and preprocess footstep-induced floor vibrations. Subsequently, we discuss the process of extracting emotion-sensitive features from these processed vibration signals to develop the general emotion recognition model.
\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{Figs/characterization.pdf}
  \caption{Placeholder}
  \label{fig:characterization}
\end{figure}
\subsubsection{Footstep-Induced Floor Vibration Collection and Preprocessing}
% We first capture the footstep-induced floor vibration signals using the vibration sensors attached to the floor. Our system uses SM-24 geophone sensors to measure vertical floor vibrations~\cite{sm24_geophone_2006}. Geophones are selected for their high sensitivity to vertical vibrations induced by footsteps. These sensors can convert vibrations into voltage signals. During the experiment, geophones are attached to the edge of the floor using wax and glue. To enhance the signal-to-noise ratio, the signals are amplified through a variable gain operational amplifier. Following the Nyquist Sampling Theorem~\cite{6773024}, the sampling rate is set at 500 Hz, considering that the structural natural frequency is below 200 Hz. 


% \subsubsection{Vibration Signal Preprocessing}
% To facilitate further processing of modeling, we preprocess the vibration signals through two main steps: 1) detecting and segmenting individual footstep signals to isolate each footstep event and 2) identifying and calibrating signal clipping aliasing to ensure precise feature extraction, thereby enhancing system accuracy and reliability. The process is initiated by identifying the peak of the continuous wavelet transform (CWT) coefficients of the vibration signals within the lower natural frequency band of the structure. A 0.35-second window is then selected around this peak to capture the essence of the individual footstep signal, assuming this duration adequately encapsulates the footstep information. This method, distinct from anomaly detection, effectively reduces misdetections in scenarios involving fast walking, where subsequent footsteps may overshadow earlier ones. Moreover, the clipping points, where signals reach the upper or lower voltage limits, are identified and calibrated via polynomial interpolation utilizing neighboring data points. This calibration step is crucial for precise frequency analysis in the following stages of feature extraction.

The vibration collection and preprocessing include three steps: 1) vibration signal collection, 2) footstep signal segmentation, and 3) signal clipping calibration. First, we collect vertical floor vibrations induced by footsteps using geophone vibration sensors. The collected vibrations are then sent to an amplifier module board to enhance the signal-to-noise ratio. Footstep segmentation is achieved by identifying the prominent peak in the wavelet transform coefficients specifically within the frequency band of dominant structural natural frequencies. This peak corresponds to the impulse force induced by a single footstep. The signal window of the average footstep duration is then extracted around this peak to isolate the footstep signal. To address signal clipping and enhance signal quality,  we first identify the clipped sections and then use polynomial interpolation to reconstruct the clipped data using the neighboring data points of the clipping sections. The clipping sections are detected when the signal reaches its upper or lower limits because clipping is due to excessive vibrations exceeding the sensor's range. Assuming the signal remains continuous, the neighboring data points of the clipping sections, which are assumed to be undistorted, carry information about the signal's original waveform. This reconstruction is accomplished by fitting a polynomial function with these neighboring points and then using this function to interpolate the data within the clipped sections, thereby achieving a continuous signal representation. In this way, we can get a continuous signal representation for the clipping sections to enhance the signal quality.

\subsubsection{Emotion-Sensitive Feature Extraction}\label{sec:feature}
To depict the information of emotional states from footstep-induced floor vibrations, we extract gait-related, structure-related, and signal-related features from the processed vibration signals. Gait-related features represent the characteristics of footsteps through gait parameters (see Table~\ref{tab:gait_feature}). Structure-related features capture information on the structural mode types associated with footsteps (see Table~\ref{tab:structure_feature}). Signal-related features characterize detailed signal properties containing nuanced gait pattern information (see Table~\ref{tab:signal_feature}).

\textbf{Gait-Related Features:} Gait-related features, referring to the gait parameters during the gait cycle, directly reflect an person's walking patterns. Gait-related features include a variety of parameters such as step frequency, double support time, peak height ratio of heel-strike and toe-off, full width at half maximum (FWHM) of these events, and various energy metrics. Each parameter plays a crucial and unique role in capturing the person's emotional states through gait patterns. For example, step frequency can increase under emotions like anxiety or happiness, while a slower step frequency might reflect sadness or fatigue~\cite{du2023spatiotemporal,lemke2000spatiotemporal,homagain2023emotional,feldman2020gait}. Similarly, double support time can help identify cautious and confident walking~\cite{xu2003emotion}. A detailed explanation of the gait-related features is shown in Table~\ref{tab:gait_feature}.

\textbf{Structure-Related Features:} To capture information about the structural mode types associated with footsteps, we investigate structure-related features utilized in structural health monitoring to extract relevant information from footstep-induced floor vibrations. Different gait patterns lead to different patterns of foot-floor contact types and ground reaction forces which results in various patterns of floor vibration mode types~\cite{dong2024ubiquitous}.
 To capture mode-type information, the structure-related features include time, frequency, and time-frequency domain features. A detailed explanation of the structure-related features is shown in Table~\ref{tab:structure_feature}.


\textbf{Signal-Related Features:}
Incorporating signal-related features from fields such as audio signal processing~\cite{eyben2010opensmile} and structural health monitoring~\cite{zhang2022vibration} can enhance the characterization of footstep-induced floor vibration signals, helping describe the complex relationship between gait patterns and emotional states. For example,  Jitter, Shimmer, and Jitter Rap quantify the variability in signal frequency and amplitude and thus can reflect the steadiness and force duration of footsteps. A detailed explanation of the signal-related features is shown in Table~\ref{tab:signal_feature}.






\textbf{Feature Characterization}
To assess the efficacy of the features and comprehend their variances across diverse emotional states, we analyze the distribution of feature values in different emotional states. Emotions are categorized into four classes: high valence high arousal (HVHA), high valence low arousal (HVLA), low valence high arousal (LVHA), and low valence low arousal (LVLA). These classes are defined based on each quadrant of the two-dimensional valence-arousal space, which is detailed in Section~\ref{sec:des_emotion}~\cite{glowinski2008technique,caridakis2006modeling,verma2017affect}. A subset of the most representative features is visually represented in Figure \ref{fig:feature_color} through a heatmap illustrating the deviations across the four emotion classes.
Under high-arousal conditions, the step frequency increases, indicating faster walking. The Full Width at Half Maximum (FWHM) of Heel-Strike and Toe-off show an increase during high valence high arousal (HVHA) scenarios. Jitter, shimmer, and jitterrap all exhibit an increase during low valence situations, reflecting a larger variance of the footstep-induced floor vibration signal. The double support time increases in low-valence situations. Additionally, the peak height ratio between heel-strike and toe-off increases during the high valence low arousal situations, indicating a tendency to lean backward. In addition, the average energy of the footstep-induced floor vibration signals increases during high-valence emotional situations, indicating a more heavy-footed walking pattern. This finding aligns with conclusions from other research in gait emotion analysis ~\cite{gross2012effort,xu2003emotion}. As depicted in Figure \ref{fig:feature_color}, the features vary across different emotion classes, demonstrating their effectiveness in extracting emotion-related information. Furthermore, different features exhibit distinct efficiency in differentiating specific emotions, emphasizing the need to combine these features for effective emotion recognition. For example, step frequency and average energy are effective in distinguishing between high and low arousal emotions, but less effective for differentiating high and low valence. Conversely, the peak ratio between heel strike (HS) and toe-off (TO) clearly separates high valence-low arousal emotions (HVLA) but shows minimal variation for other emotions.



\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{Figs/feature_color_v4.pdf}
  \caption{Heatmap of Normalized Feature Deviations across Emotion Classes. Each cell indicates the deviation from the overall mean for a given feature under specific emotional conditions. Positive values (towards 1.00) suggest that the feature increases in the corresponding emotion classes, while negative values (towards -1.00) denote that the feature decreases in the corresponding emotion classes. The effectiveness of these features is evident in their varying performance across different emotion classes. }
  \label{fig:feature_color}
\end{figure}

In summary, we develop an emotion-sensitive feature set that includes gait-related features, structure-related features, and signal-related features to represent the complex relationship between emotion and footstep-induced floor vibrations. These features are collectively utilized for the comprehensive analysis of inferring emotional states.
% \subsection{Emotion Recognition Modeling}
% After extracting emotion-sensitive features from footstep-induced floor vibration signals, we construct an emotion recognition model to infer individuals' emotions. Initially, this involves developing a general emotion recognition model. Subsequently, if specific information about the target individual is available, we can enhance this by implementing a person-specific emotion recognition model. This adaptation integrates information from the target individual, thereby optimizing the model's performance for that particular person.
\subsection{General Emotion Recognition Development}
\label{sec:general_model}

% In this section, we develop a general emotion recognition model that represents the preliminary relationship between emotion and footstep-induced floor vibrations in the situation when we don't have the target person's floor vibrations data. This model serves as a baseline model for emotion recognition. To mitigate the potential model overfitting caused by the limited dataset, we simplify the complexity of the model through iterative pruning by cutting down the least important parameters within the model.
% I rewrite this paragraph shown below. Because that there are too many modifications, thus I rewrite instead of modification on the previous one.
In this section, we develop a general emotion recognition model using the extracted emotion-sensitive features. Without the input of specific information about the target person’s (i.e., the individual whose emotions we aim to recognize) footstep-induced floor vibrations, the general model takes all people in the training set with equal weight during training to establish a preliminary relationship between emotions and footstep-induced floor vibrations. To mitigate the potential model overfitting challenge caused by the limited dataset, we simplify the complexity of the model by cutting down the least important parameters within the model through iterative pruning. The development of the general emotion recognition model provides the basis for subsequent personalization.

\subsubsection{General Emotion Recognition Modeling}
We develop a general emotion recognition model to build a preliminary relationship between emotion and footstep-induced floor vibrations before inputting specific information about the target person’s footstep-induced floor vibrations. 
The model architecture is illustrated in Figure~\ref{fig:iteration_prune_2}. The extracted emotion-sensitive features, which include gait-related, structure-related, and signal-related features as described in Section~\ref{sec:feature}, are regrouped into three types based on their data format: singular value features, one-dimensional sequential features, and two-dimensional image-like features. Different types of neural network layers are employed based on the distinct properties of these features' data formats. For singular value features, we use fully connected layers to decode information because these layers contain separate parameters for each input feature value, enabling the direct modeling between the feature and the output. Sequential features have dependencies across time steps. So they are processed through long short-term memory (LSTM) layers, which excel at capturing the temporal dependencies and deciding which data to retain or omit over sequences via the gating mechanism~\cite{hochreiter1997long}. Two-dimensional time-frequency spectrum image features, such as those derived from continuous wavelet transforms (CWT), are analyzed with convolutional layers. The convolutional layers are chosen because they can preserve the spatial and temporal relationships within the time-frequency spectrum image features. The output from each processing layer is combined and input into a multilayer perceptron with two fully connected layers, which outputs valence and arousal scores for the emotion score estimation task or emotion class labels for the emotion classification task. In addition, dropout layers are incorporated after the concatenation to reduce the overfitting caused by the noise and fluctuations within the training data~\cite{srivastava2014dropout}. The mean absolute error (MAE) is selected as the loss function for the emotion score estimation task due to its ability to provide a linear quantification of prediction errors, which is essential for regression-based tasks~\cite{willmott2005advantages}. For the emotion classification task, the cross-entropy loss is used because of its label-invariant nature~\cite{song2022learning}.
\begin{figure}[ht] 
  \centering
  \includegraphics[width=\linewidth]{Figs/method_structure_v4.pdf}
  \caption{Emotion Recognition Neural Network Architecture. Three types of features are regrouped based on their data structure—singular value, 1D sequential, and 2D image-like features to utilize distinct neural network layers—Dense, LSTM, and Convolutional layers for each feature type. The processed features are then fused in a concatenated layer, enabling the final dense layers to determine the emotion, quantified by valence and arousal scores. }
  \label{fig:iteration_prune_2}
\end{figure}


\subsubsection{Model Complexity Simplification}
\label{sec:iterative_prune}

% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=0.8\linewidth]{Figs/iteration_prune_v4.pdf}
%   \caption{General emotion recognition modeling with iteration pruning.}
%   \label{fig:iteration_prune}
% \end{figure}



% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=\linewidth]{Figs_v2/method_pruning.pdf}
%   \caption{Iterative Pruning Process for Neural Network Simplification. Initial training occurs during the burn-in period before pruning begins to acquire the initial trained parameter values, which are used to assess the importance of each parameter. Pruning commences at the iterative pruning period, progressively eliminating non-critical parameters until the end of this period, as depicted by the descending line graph. During the consolidation period, the network's refined architecture is further trained to enhance performance while maintaining the reduced parameter set.}
%   \label{fig:iteration_prune_3}
% \end{figure}

We simplify the emotion recognition model by cutting down the least important parameters within the model through iterative pruning to mitigate model overfitting caused by the limited dataset size. The original feature set spans over 10,000 dimensions, suggesting a requirement for a dataset size at least ten times this number, or over 100,000 footstep samples, to train the network, as indicated by ~\cite{alwosheel2018your,baum1988size}. This requires 40 hours of continuous walking, not including the time allocated for emotion elicitation. The limited dataset can lead to model overfitting. However, conducting human experiments to gather such a vast dataset is prohibitively expensive and logistically challenging. % Emphasis the innovation of our work.
To address this challenge, we develop the model complexity simplification method using the iterative pruning method which iteratively cuts down the least important parameters within the neural network during the training process. The iterative pruning method was proven effective in cutting down parameters within the network for reducing the computational time while keeping the model performance ~\cite{ge2020compressed}. In this work, iterative pruning is used for model simplification to mitigate overfitting which improves the model performance in the situation with a limited dataset.
 The iterative pruning algorithm includes three phases: The initial phase involves training the network to obtain baseline parameter values without any reduction, providing a foundation for evaluating parameter importance. Subsequently, the second phase involves pruning the least important parameters after each training epoch, systematically eliminating non-essential parameters until this phase concludes. In the final phase, pruning stops, and the network is further trained with the pruned architecture to improve performance. The number of epochs of each phase is a hyperparameter selected through the grid search method. After iterative pruning, we obtain a general emotion recognition model that can estimate emotion (valence and arousal scores) from the input features extracted from the footstep-induced floor vibrations with fewer parameters.
 
\subsection{Personalized Emotion Recognition Development}


In this section, we develop a personalized emotion recognition model with the footstep-induced floor vibrations from the target person (i.e., the individual whose emotions we aim to recognize). The personalized emotion recognition model achieves better performance for the target person given the incorporated target person's footstep-induced floor vibrations. The personalization process contains two steps. First, we assess the gait similarity between the target person and the people in the training dataset and quantify the similarity using the gait similarity indices. Subsequently, we personalize the emotion recognition model by fine-tuning with these gait similarity indices as weights assigned to the training data in the loss function. During the fine-tuning, the model multiplies the loss by the sample’s weight instead of treating each sample’s loss equally. This allows the samples with higher weights to contribute more to the fine-tuning process. As a result, the model updates its parameters more significantly in response to the samples of higher weights, which are more similar to the target individual’s gait samples.


\subsubsection{Gait Similarity Comparison}
\label{sec:gsc}
In this subsection, we compare the gait similarity between the people in the training set and the target person based on their footstep-induced floor vibrations, quantifying this similarity using the gait similarity indices. The gait similarity indices serve as weights assigned to the training samples, facilitating further personalization of the emotion recognition model.
The gait similarity indices calculation steps are detailed as follows:

\textbf{A. Euclidean Distance Calculation:} For each training person, we first calculate the Euclidean distance between all sample pairs comprising one footstep sample from the target person ($P_T$) and another from the training person ($P_i$, where i = 1, 2, ..., n). These distances are calculated using embeddings of the samples which correspond to the concatenated layer values obtained from the general emotion recognition model built in the general emotion modeling procedure (details in Section~\ref{sec:iterative_prune}). We assume that these concatenated layers effectively represent essential gait information, as they integrate data across all feature types. The Euclidean distance between the $k_1$-th sample embedding ($E_T^{k_1}$) from the target person and the $k_2$-th sample embedding ($E_i^{k_2}$) from training person $P_i$ is calculated as:
$$d(E_T^{k_1}, E_i^{k_2}) = ||E_T^{k_1} - E_i^{k_2}||_2$$
In this formula, $||\cdot||_2$ signifies the L2 norm, which calculates the Euclidean distance to represent the dissimilarity of two embedding vectors~\cite{dokmanic2015euclidean}. The L2 norm is obtained by taking the square root of the sum of the squared differences between corresponding elements of $E_T^{k_1}$ and $E_i^{k_2}$. The Euclidean distances indicate the similarity between pairs of footstep samples, with shorter distances corresponding to greater similarity.
% Section~\ref{sec:iterative_prune} describes obtaining a general emotion model that establishes a preliminary relationship between emotions and footstep-induced floor vibrations. Moreover, a concatenated layer in this model identifies a latent embedding encapsulating gait pattern information from the vibrations. Assuming this layer serves as an effective embedding of essential gait information, gait similarity is quantified by the reciprocal of the average Euclidean distance between the embeddings of the target and training individuals' gait samples. A smaller distance signifies greater similarity, thus indicating a higher gait similarity index. The calculation steps are detailed as follows:

% 1) Euclidean Distance Calculation: The Euclidean distance between each pair of target gait embeddings ($E_T$) from the target individual ($P_T$) and training gait embeddings ($E_i$) from the training individual ($P_i$, where i = 1, 2, ..., n) for specific samples is computed as follows:
% $$d(E_T^{k_1}, E_i^{k_2}) = ||E_T^{k_1} - E_i^{k_2}||_2$$

% In this formula, $||\cdot||_2$ signifies the L2 norm, which calculates the Euclidean distance. Here, $d(E_T^{k_1}, E_i^{k_2})$ represents the distance between the $k_1$-th sample from the target individual and the $k_2$-th sample from training individual $P_i$. The L2 norm is obtained by taking the square root of the sum of the squared differences between corresponding elements of $E_T^{k_1}$ and $E_i^{k_2}$.

\textbf{B. Average Euclidean Distance:} Considering the intra-person gait variability, we then average the Euclidean distances for all samples from the target and the training person to reduce the impact of any outlier footsteps or noise, leading to a more reliable and stable similarity representation. This averaging approach mitigates the potential distortion caused by outlier samples, ensuring a more stable weight normalization process. The average Euclidean distance ($D_{i}$) is calculated as follows: 
\[D_{i} = \frac{1}{K_1 \times K_2}\sum_{k_1=1}^{K_1}\sum_{k_2=1}^{K_2} d(E_T^{k_1}, E_i^{k_2})\]

In this formula, $K_1$ denotes the number of gait samples from the target person, and $K_2$ signifies the number of training people, $P_i$. The average Euclidean distances ($D_{i}$) indicate the overall similarity of the target person's ($P_T$) gait patterns and the training person's ($P_i$) gait patterns, with smaller $D_i$ values for greater similarity.

\textbf{C. Gait Similarity Index (GSI) Calculation:} To ensure that a higher GSI corresponds to a greater similarity in gait patterns, the Gait Similarity Index (GSI) is established as the normalized inverse of this average distance ($D_i$):
\[\widehat{GSI_i} = \frac{1}{D_{i}}, GSI_i = \frac{\widehat{GSI_i}}{max_i(\widehat{GSI_i})}\]

Normalization is executed by dividing each GSI by the maximum GSI observed across the training people, constraining similarity indices to a range between 0 and 1, thereby facilitating weight assignment. Similar gait patterns usually have smaller Euclidean distances, thus corresponding to larger GSI values.

\subsubsection{Personalized Emotion Recognition Modeling}
After assessing the gait similarity indices (GSI) between the target person and the individuals in the training set, we personalize the general emotion recognition model (see Section~\ref{sec:general_model}) through fine-tuning. During this process, the parameters from the pruned general model are utilized as the initial model settings. Training samples are weighted according to their GSI values, meaning that during loss function computation, each sample's loss is adjusted by its corresponding weight. Consequently, data from individuals with gait patterns similar to the target person receive higher weights, thus improving model performance for the target person by concentrating training on similarly distributed gait patterns.



==> Sections/not_used/04Evaluation.tex <==
\section{Real-World Walking Experiment Evaluation}
To evaluate EmotionVibe's performance, we conduct a real-world walking experiment, collecting a dataset that includes footstep-induced floor vibrations and corresponding emotion labels from 30 participants. We analyze data from 20 participants, excluding those with erroneous data because they kicked sensors as they walked and people who are rarely affected by the emotion elicitations. Our system achieves mean absolute errors of 1.11 for valence score estimation and 1.07 for arousal score estimation, within a score range of 1 to 9, representing a 22.4$\%$ error reduction compared to the baseline method. Furthermore, our system achieves a 60$\%$ accuracy and a 0.59 F1 score for emotion classification in a four-class emotion classification task encompassing High Valence High Arousal (HVHA), High Valence Low Arousal (HVLA), Low Valence High Arousal (LVHA), and Low Valence Low Arousal (LVLA).
% (Out of the 30 individuals who participated in the experiment, 20 provided valid and available data.) 
% The evaluation was carried out in two scenarios. In the first scenario, the general emotion recognition model is evaluated with randomly shuffled data split into training, validation, and test sets. Our method achieved a mean absolute error of 1.23 for both valence and arousal score estimation. The second scenario involved a leave-one-subject-out approach for evaluating the person-specific emotion recognition system. In this approach, one person's data was used as the test set while the data from the remaining individuals served as the training and validation sets. Employing a person-specific emotion recognition model, we achieved a mean absolute error of 1.54 for both valence and arousal score estimation.


\subsection{Real-World Walking Experiment Setup}
We conduct the real-world walking experiment on a wooden platform in a laboratory setting with 30 healthy students from Stanford University, including 14 males and 16 females. The wooden platform, with dimensions of 7.31 meters in length and 2 meters in width, is equipped with four SM-24 geophone sensors ~\cite{sm24_geophone_2006} attached to the floor's edge using wax and glue, as illustrated in Figure~\ref{fig:experiment}. Following the Nyquist Sampling Theorem~\cite{6773024}, the sampling rate is set at 500 Hz, considering that the structural natural frequency is below 200 Hz.  All experiments are carried out in compliance with approved Institutional Review Board (IRB) protocols (Stanford IRB Protocol: 54912).
% The experiment took place indoors on a wooden platform measuring 7.31m x 2m. Four SM-24 geophone sensors, securely attached to the floor using wax and glue, were used to capture the footstep-induced floor vibration signals, with a sampling rate of 500 Hz. To avoid interfering with the participants' walking process, the sensors were positioned at the platform's edge. Figure ~\ref{fig:experiment} illustrates the specific sensor locations. All experiments were conducted following approved IRB protocols.

In the experiment, we use various music clips and light stimuli to evoke distinct emotions, as detailed in Table~\ref{tab:emotion_stimulus}. Eight pairs of emotion elicitation were designed to correspond to four target emotional states: high valence high arousal, high valence low arousal, low valence high arousal, and low valence low arousal. The selected music clips were obtained from the PUMS database, with their efficacy in influencing human emotions previously validated in a study by  ~\cite{warrenburg2021pums}. Light stimuli include a shining light for high arousal scenarios, bright white for high valence low arousal, colorful shining colors for high valence high arousal, red and yellow for low valence high arousal, and dark blue for low valence and low arousal situations. The effectiveness of light stimuli in eliciting emotions is supported by existing literature~\cite{wilson1966arousal,elliot2015color,valdez1994effects,iskra2008daytime}. For instance, bright colors like yellow, orange, pink, and red are associated with motivation and energy, while cool colors like green, blue, and violet have a calming effect~\cite{elliot2015color,wilson1966arousal}. Both saturation and brightness play a role in influencing emotions, suggesting that color intensity and lightness can affect emotional responses~\cite{valdez1994effects}. Intermittent bright light pulses have been shown to have immediate and lasting alerting effects, increasing arousal in people ~\cite{iskra2008daytime}. The Govee RGB LED Strip is used to create varied lighting conditions, while music clips are delivered to participants using AirPods.

\begin{table}[ht]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{Emotion Type}                                  & \multirow{2}{*}{Musical Pieces}                                            & \multirow{2}{*}{Light Type} \\ \cline{1-2}
Valence               & Arousal               &                           &                                                                            \\ \hline
\multirow{2}{*}{High} & \multirow{2}{*}{High} & Peer Gynt   Suite No. 1, Op. 46, Mvt 4, In the Hall of the Mountain   King & Colorful, Shining           \\ \cline{3-4} 
                      &                       & Prelude and Fugue No. 15 BWV 860, I.   Prelude in G Major                  & Colorful, Shining           \\ \hline
\multirow{2}{*}{High} & \multirow{2}{*}{Low}  & Nocturne No. 2, Op. 9 in E Flat   Major                                    & White, Steady               \\ \cline{3-4} 
                      &                       & Blue in Green                                                              & White, Steady               \\ \hline
\multirow{2}{*}{Low}  & \multirow{2}{*}{High} & Dracula, Vampire Hunters                                                   & Red/ Yellow, Shining        \\ \cline{3-4} 
                      &                       & High-Wire Stunts                                                           & Red/ Yellow, Shining        \\ \hline
\multirow{2}{*}{Low}  & \multirow{2}{*}{Low}  & Adagio in G Minor                                                          & Dark Blue, Steady           \\ \cline{3-4} 
                      &                       & The Seven Last Words of Jesus Christ,   Op 51, Mvt 3                       & Dark Blue, Steady           \\ \hline
\end{tabular}%
}
\caption{Emotion Elicitation Set for the Real-World Walking Experiment. The table lists eight musical pieces with corresponding light types to evoke specific emotional states, categorized by different emotion classes.}
\label{tab:emotion_stimulus}
\end{table}

The experimental procedure is as follows: 
\begin{enumerate}
    \item The participant is guided to walk on the platform for 2 to 3 minutes while experiencing their initial emotions.
    \item The participant is guided to complete the Self-Assessment Manikin (SAM) survey scale (see Appendix)~\cite{bradley1994measuring}. They should rate their emotional valence and arousal on a scale from 1 to 9.
    \item The participant is exposed to a set of emotional elicitation, randomly selected from the eight categories outlined in Table ~\ref{tab:emotion_stimulus}, for 1 minute.
    \item The participant is guided to continue walking on the platform for another 2 to 3 minutes. This walk should be accompanied by music and lighting corresponding to the previously presented emotional elicitation.
    \item The participant is guided to complete the SAM survey scale again to assess their emotional state during the walk and evaluate the impact of the emotional stimuli. Details and instructions for this assessment are provided in the Appendix.
    \item Repeat steps 3 to 5 with alternative emotional elicitation. This is done 8 times, each with a different set of stimuli from the specified categories.
\end{enumerate}

During the experiment, each participant completes a total of nine walking trials, with each trial lasting 2 to 3 minutes. 
We exclude the data of people who either did not complete the experiment or kicked the sensors while walking. Additionally, we eliminated data from participants whose average feedback score was lower than 2, indicating that our emotional stimulus rarely influences them. Finally, we get 37,001 footstep samples from the four sensors in the dataset for evaluation.

\begin{figure}[ht]
  \centering\includegraphics[width=\linewidth]{Figs/experiment_v2.pdf}
  \caption{Real-World Walking Experiment Setup. In the experiment, participants are initially exposed to specific types of emotion elicitation (music and light) before being instructed to walk on the platform while the elicitation continues. Sensors placed on the floor capture the vibrations induced by footsteps during walking.}
  \label{fig:experiment}
\end{figure}
\subsection{Implementation Details}
\subsection{Dataset Overview and Effectiveness Validation}
The emotion elicitation evaluated impact scores (responses to the third question presented in the Appendix) from participants and the diversity of emotion labels within the dataset confirm that our emotional stimuli effectively influenced these participants' emotions and that the data collected is diverse, including a wide range of emotions.
Figure~\ref{fig:feedback} and Figure~\ref{fig:data_distribution} demonstrate that our experiment elicited a moderately strong average effect on participants' emotions with data from diverse emotional situations spanning the entire valence-arousal 2D space. To assess the efficacy of our emotional stimuli, participants were asked to report on the impact of these stimuli on their emotional states during the experiment, after each walking trial. These reports are used to exclude participants whose emotional responses did not vary significantly throughout the experiment, indicating that our emotional stimuli were ineffective for them. Subsequently, the average feedback score from the remaining 20 participants is presented in Figure~\ref{fig:feedback}. The overall average emotion elicitation evaluated impact score of 5.11 suggests a moderately strong influence of our emotional stimuli on participant emotions. Furthermore, it is crucial to ensure the dataset encompasses a broad range of emotion types. Figure~\ref{fig:data_distribution} displays a bubble plot illustrating the diverse emotional states captured in our dataset, thereby confirming the diversity of our dataset.
%% figure 1: feedback score distribution, emotion range
%% figure 2: emotion score distribution in the valence and arousal space.
% \begin{figure}[ht]
%     \centering
%     \begin{minipage}{0.45\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{Figs/feedback.pdf} % First figure
%         \caption{Impact of Emotional Stimuli on Participants (Feedback Scores)}
%         \label{fig:feedback}
%     \end{minipage}\hfill
%     \begin{minipage}{0.45\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{Figs/data_distribution_v2.pdf} % Second figure
%         \caption{Distribution Density of Emotion Scores within the Dataset (Size of the point is proportional to data density)}
%         \label{fig:data_distribution}
%     \end{minipage}
% \end{figure}

\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.40\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Figs_v2/feedback_v3.pdf}
        \caption{}
        \label{fig:feedback}
    \end{subfigure}\hfill
    \begin{subfigure}{0.47\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Figs_v2/data_distribution_v3.pdf}
        \caption{}
        \label{fig:data_distribution}
    \end{subfigure}
    \caption{Participant Evaluated Impact Scores and Emotion Scores Distribution Demonstrating the Efficacy of Our Emotional Stimulus and the Diversity of Emotions in the Dataset. (a) Bar chart representing the evaluated impact scores from 20 participants, with the average score denoted by a horizontal line at 5.11, suggesting a moderate response to the emotion elicitation. (b) The bubble plot of the emotion scores distribution depicts the density of data points across the valence-arousal space, indicating a varied emotional impact rather than a concentration in a specific region.}
    \label{fig:data_experiemnt}
\end{figure}
\subsection{Emotion Recognition Results of EmotionVibe}
We evaluate the performance of EmotionVibe described in Section 3 using the real-world walking experiment data from 20 participants which includes 37,001 footstep samples. Our system achieves up to 1.11 for valence score estimation and 1.07 for arousal score estimation (score range: [1, 9]), representing a 22.4$\%$ error reduction compared to the baseline method. The baseline model utilizes only gait-related features, which represent parameters derived from prior research on gait patterns and emotions, without model simplification using iterative pruning or personalization used in EmotionVibe.

\subsubsection{Valence / Arousal Score Estimation Results}
EmotionVibe is evaluated using the dataset collected from the real-world walking experiment, which includes data from 20 participants and 37,001 footstep samples. The evaluation process is conducted 20 times. Each time we take a different participant as the target person. Subsequently, the average of these 20 evaluations serves as the final estimation result.  For each participant's evaluation, 60$\%$ of their data (approximately 10 minutes of walking data encompassing 90 traces with 4 sensors) is allocated to the training and validation sets, with the remaining 40$\%$ for the test set. This division ratio is determined by balancing the time required to collect sufficient data from each participant against the necessity for a data volume that enhances model performance. The implications of varying this data allocation ratio are further explored in Section~\ref{sec:sys_cha_2}. Data for training and validation are randomly divided in a 9:1 ratio, including all the data from training people and 60$\%$ data from the target person for validation. We keep data from the same walking trace together during splitting, ensuring that data from the same trace are not fragmented across different sets to prevent potential data leakage into the test set. Model hyperparameters are selected via the grid search method, and the model achieving the best validation performance is used for testing. After obtaining the estimation scores for the test set, we compute the median of the emotion score estimations from footsteps in each trace to derive the overall emotion estimation for that trace. This methodology effectively mitigates the impact of extreme value estimations and reduces the variance in emotion estimation. The ground truth for these estimations is established using the emotion scores collected from participants through the Self-Assessment Manikin (SAM) survey scale. 

EmotionVibe achieves mean absolute errors of 1.11 for valence score estimation and 1.09 for arousal score estimation, demonstrating a significant 22.4$\%$ error reduction compared to the baseline method (see Figure~\ref{fig:feature_comp_2}).
Figure~\ref{fig:data_scatter} presents a scatter plot comparing predicted scores against ground truth for valence and arousal, showing moderate linear correlations with the Pearson correlation score of 0.612 and 0.695, respectively. As a reference, the state-of-the-art emotion recognition using EEG sensors reports a mean absolute error of 0.06 (on a scale of 0 to 1, equivalent to MAE of 0.48 on a 1 to 9 scale) and a Pearson correlation of 0.8 between the EEG-based emotion score and the reported emotion score, utilizing a complex combination of EEG signal channels~\cite{galvao2021predicting}. Despite the challenges of information loss and the inherent uncertainty of human gait behaviors, our system yields relatively accurate estimations.

% Explanation of the baseline models
The effectiveness of emotion-sensitive feature extraction, iterative pruning, and personalization are proved by the reduced emotion recognition error, as illustrated in Figure~\ref{fig:feature_comp_2}. To evaluate the effectiveness of personalization, we compared the general emotion recognition model (before personalization) with our method. The results indicate an 11.4$\%$ reduction in error by personalization (see Figure~\ref{fig:feature_comp_2} (a)). To evaluate the effectiveness of iterative pruning, we compare the results of the method using iterative pruning (our method) with both a non-pruned model and the method utilizing feature selection instead of iterative pruning for model simplification which selects the top features with the highest maximal information coefficient (MIC) correlation scores (Feature Selection Method). Our method shows the best performance, indicating the effectiveness of model simplification through iterative pruning (see Figure~\ref{fig:feature_comp_2} (b)). Moreover, by comparing with models trained on a single feature type and feature ablation studies, we prove the indispensability of each feature and the necessity of combining these features for optimal emotion recognition performance. Figure~\ref{fig:feature_comp_2} (c) shows that while these models do not perform as well as our method, they still achieve comparatively low error rates, indicating their utility. Figure~\ref{fig:feature_comp_2} further reveals that the omission of any feature results in increased estimation error, underscoring the necessity of feature combination for optimal emotion recognition performance.


% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=0.5\linewidth]{Figs/comparison_ap.pdf}
%   \caption{General model result: Comparison of overall baseline and Adaptive Pruning}
%   \label{fig:result}
% \end{figure}
% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=\linewidth]{Figs_v2/result_comparison_boxplot.pdf}
%   \caption{Boxplot Comparison of the Emotion Estimation Error between Various Methods. Compared to traditional feature selection, single-feature models, and feature ablation tests, our method maintains the lowest error, indicating that our iterative pruning simplifies the model without compromising performance. In addition, it suggests the necessity of the combined feature approach for accurate valence and arousal estimation.}
%   \label{fig:feature_comp}
% \end{figure}

% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=\linewidth]{Figs_v2/result_compare_v4.pdf}
%   \caption{Comparison of the Mean Absolute Errors in Emotion Score Estimation between Various Methods. Compared to the general emotion recognition method, method without pruning, traditional feature selection, single-feature models, and feature ablation test models, our method maintains the lowest error, indicating that our iterative pruning simplifies the model without compromising performance. In addition, it suggests the necessity of the combined feature method for accurate valence and arousal estimation.}
%   \label{fig:feature_comp_2}
% \end{figure}

\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Figs_v2/scatter_valence.pdf}
        \caption{}
        \label{fig:valence_corr}
    \end{subfigure}\hfill
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Figs_v2/scatter_arousal.pdf}
        \caption{}
        \label{fig:arousal_corr}
    \end{subfigure}
    \caption{Scatterplots of Predicted and Ground Truth Scores for Emotion Estimation. (a) Valence prediction versus actual with a Pearson Correlation of 0.612. (b) Arousal prediction versus actual with a Pearson Correlation of 0.695. Each point represents a data pair in the evaluation.}
    \label{fig:data_scatter}
\end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{Figs_v2/result_compare_v4.pdf}
  \caption{Evaluation of the Effectiveness of Our Method in Emotion Recognition Error Reduction. (a) Our method outperforms the general emotion recognition method, indicating the effectiveness of personalization. (b) Our method outperforms both non-pruned models and models simplified using feature selection, underscoring the effectiveness of our iterative pruning technique. (c) Our method yields the lowest emotion recognition error when compared to models utilizing a single feature type, demonstrating the importance of feature integration. (d) In feature ablation tests, our method consistently shows reduced error rates, indicating the effectiveness of feature combinations.}
  \label{fig:feature_comp_2}
\end{figure}

% \begin{figure}[ht]
%   \centering
%   % First figure
%   \begin{minipage}[b]{0.45\linewidth}
%     \includegraphics[width=\linewidth]{Figs/scatter_valence.pdf}
%     \caption{Valence Estimation (Pearson Correlation score: 0.550)}
%     \label{fig:valence_corr}
%   \end{minipage}
%   \hfill % This adds a little space between the figures
%   % Second figure
%   \begin{minipage}[b]{0.45\linewidth}
%     \includegraphics[width=\linewidth]{Figs/scatter_arousal.pdf}
%     \caption{Arousal Estimation (Pearson Correlation score: 0.653)}
%     \label{fig:arousal_corr}
%   \end{minipage}
% \end{figure}



% In our emotion estimation process, we adopt the median value of all the emotion scores obtained from the footstep signals within each trial as the estimated emotion for that trial. This smoothing technique at the trial level is based on the assumption that individuals' emotions remain consistent throughout each trial. Figure ~\ref{fig:trace_stp} illustrates the implementation of this trial-level smoothing approach, which effectively reduces both the error in emotion estimation and the variability of the errors. Implementing the trial smoothing technique results in a decrease in the mean absolute error from 1.31 and 1.36 to 1.23 and 1.23 respectively, and a decrease in the median error from 1.64 and 1.91 to 0.92 and 0.51 for valence and arousal score estimation respectively.
% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=0.5\linewidth]{Figs_v2/trace_stp_v2.pdf}
%   \caption{Comparative boxplot of estimation errors in valence (black) and arousal (gray) at footstep and trial levels. The trial level shows lower errors (median error of 0.92 for valence and 0.51 for arousal), indicating more precise estimations than the footstep level.}
%   \label{fig:trace_stp}
% \end{figure}

% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=\linewidth]{Figs/feature_ablation.pdf}
%   \caption{Feature Ablation Test (Using Adaptive Pruning)}
%   \label{fig:feature_abalation}
% \end{figure}
\subsubsection{Emotion Classification Results}
Additionally, EmotionVibe exhibits good performance, comparable to existing conventional gait-based emotion recognition systems, on the emotion classification task. This task aims to estimate the emotion types (High Valence High Arousal (HVHA), High Valence Low Arousal (HVLA), Low Valence High Arousal (LVHA), and Low Valence Low Arousal (LVLA)~\cite{cao2020eeg}). Participants' scores from the SAM survey scale are used to determine the classes, with scores lower or equal to 5 categorized as low valence/arousal and scores higher than 5 categorized as high valence/arousal. For the classification task, the only modification made to the model is changing the last layer to a dense layer with 4 units and applying softmax activation, with the loss function set to cross-entropy loss. EmotionVibe achieves 60$\%$ accuracy for emotion classification with the F1 score of 0.54. The confusion matrix is shown in Figure~\ref{fig:unbalance}. The model tends to classify samples into the HVLA (High Valence, Low Arousal) class, attributed to an imbalanced dataset. As depicted in Figure~\ref{fig:data_distribution}, the HVLA class contained a disproportionately higher number of samples compared to the other three classes. To mitigate this imbalance, we adopted a dataset-balancing technique that assigns class weights to the training samples. The ratio of the total number of samples to the number of samples in that specific class determines the class weight for each class. The class weights are applied in calculating the loss function to emphasize the importance of samples from less represented classes, effectively increasing the F1 score to 0.59 while maintaining an accuracy of 60$\%$.

\begin{figure}[ht]
  \centering
  % First subfigure
  \begin{subfigure}[b]{0.45\linewidth}
    \includegraphics[width=\linewidth]{Figs_v2/cm_unbalance.pdf}
    \caption{}
    \label{fig:unbalance}
  \end{subfigure}
  \hfill % This adds a little space between the subfigures
  % Second subfigure
  \begin{subfigure}[b]{0.45\linewidth}
    \includegraphics[width=\linewidth]{Figs_v2/cm_balance.pdf}
    \caption{}
    \label{fig:balance}
  \end{subfigure}
  
  \caption{Comparative Analysis of Confusion Matrices for Emotion Classification. The matrices display classification results for four emotional states: High Valence High Arousal (HVHA), High Valence Low Arousal (HVLA), Low Valence High Arousal (LVHA), and Low Valence Low Arousal (LVLA). (a) illustrates the results without dataset balancing, yielding an F1 score of 0.54. (b) shows improved classification accuracy after balancing the dataset, as evidenced by an increased F1 score of 0.59. The matrices indicate a higher true positive rate for each emotional state post-balancing, demonstrating the impact of dataset distribution on classification performance.}
\end{figure}
\subsection{System Characterization}
In this subsection, we assess EmotionVibe's performance consistency across different individuals and evaluate its effectiveness with varying sample sizes from the target person.

% \subsubsection{Effect of Individual Variability on System Performance Consistency}
\subsubsection{System Performance Consistency Across Different Individuals}

We examine the performance consistency of EmotionVibe across different individuals and observe a consistent error reduction through personalization for the majority of participants, as illustrated in Figure~\ref{fig:personcompare}. The system demonstrates its lowest estimation error for Person 18, with a mean absolute error (MAE) of 0.52 (valence score estimation error: 0.48, arousal score estimation error: 0.56). Conversely, the worst performance is recorded for Person 4, with an MAE of 1.9 (valence score estimation error: 2.18, arousal score estimation error: 1.68). Notably, even in the least favorable case, our method's MAE remains below 2 within a range of 1 to 9, indicating a consistently high level of performance in emotion estimation tasks. Furthermore, the system exhibits significant error reduction for the majority of people, with the most notable improvement observed for Person 6, where the MAE decreases from 2.07 to 1.39. However, the system does not reduce the error for Persons 4 and 16, potentially due to their unique gait patterns, which lack similar samples in the whole training dataset. Specifically, our analysis revealed that Person 4 wore boots with a particularly hard heel, and Person 16 was the only participant wearing high heels, distinguishing their gait patterns from the rest of the participants. These outlier gait patterns affect the accuracy of the gait similarity index score estimation, thus affecting the model's performance. A potential solution could involve enriching the dataset with more diverse data, including examples of gait patterns of high heels and hard-heeled boots.

% \subsubsection{Effect of Proportion of Target Person's Data in the Training Set on System Performance}
\subsubsection{System Performance with Varying Target Person Samples}
\label{sec:sys_cha_2}
% Effect of target person's data portion in the training set on system performance
We assess EmotionVibe's performance to variations in the number of samples from the target person included in the training dataset. We note a decrease in emotion estimation error as the quantity of input data from the target person increases, as depicted in Figure~\ref{fig:fewshot}. Remarkably, even without incorporating any data from the target person into the training set, our system achieves mean absolute errors (MAE) of 1.54 and 1.54 for valence estimation and arousal estimation, respectively. When the training set is enriched with approximately 90 walking traces from the target person, the system's performance improves, resulting in a reduced MAE of 1.09, with valence and arousal score estimation errors of 1.11 and 1.07, respectively. In this context, each trace refers to data collected by a single sensor, documenting the subject walking once across a 7.31m platform (around 7 seconds). With four sensors deployed, it is feasible to gather 90 walking traces within approximately 10 minutes of continuous walking. 
% The previous evaluation takes 90 walking traces from the target person in the training considering the trade-off between the time required for data collection and the necessity for a data volume that enhances model performance.

% \subsubsection{Emotion Estimation of the Person Specific Emotion Recognition}

% The evaluation of person-specific emotion recognition is conducted in two scenarios. In the first scenario, none of the target person's data is included in the training set. In the second scenario, we incrementally add a small amount of data from the target person to the training set and assess the model's performance using varying numbers of the target person's data.

% In the first scenario, we employ the leave-one-subject-out method for each individual within a dataset comprising 20 participants' data. The average error of the 20 models is calculated (one for each person). During each iteration, one person's data is withheld as the test set, while the remaining individuals' data is randomly divided into a training set and validation set at a ratio of 9:1. Initially, the general emotion recognition model is trained using iteration pruning technique on the training set. Subsequently, the hidden layer of the general emotion recognition model is utilized to compute the similarity index between each person in the training set and the target person, achieved by calculating the Euclidean distance between the hidden layers for different sample inputs. The general emotion recognition model is then fine-tuned using the similarity index assigned as weights to the training data. In this scenario, the baseline model is defined as the general emotion recognition model before the fine-tuning process. The results demonstrate that our method achieves enhanced performance with lower error compared to the baseline method, as depicted in Figure ~\ref{fig:personspecific}.

% In the second scenario, based on the first scenario, we divided the data from the target person into a training set and a test set. For the target person's data in the training set, a weight of 50 was assigned (5 times the weight of the largest weight assigned to other individuals in the training set, determined through grid search). Similar to the approach used in the first scenario, we developed a person-specific emotion recognition model by incorporating more information about the target person. The results were obtained by averaging the performance of 20 models (one model for each person). As shown in Figure ~\ref{fig:fewshot}, as we gradually added data from the target person to the training set, the error in emotion estimation progressively decreased, indicating better model performance. When approximately 90 walking trials' data from the target person were included, the model achieved a mean absolute estimation error of 1.09 (1.11 for valence score estimation, 1.07 for arousal score estimation), representing an 11.4 $\%$ reduction in error compared to the general emotion recognition model (Mean absolute error: 1.23). It should be noted that while the general emotion recognition model can classify emotions for multiple individuals, the person-specific emotion recognition model only yields superior performance for the corresponding target person.
\begin{figure}[ht]
  \centering
  \includegraphics[width=0.7\linewidth]{Figs_v2/person_compare_with_avg_lines.pdf}
  \caption{Comparison of Mean Absolute Errors (MAE) for emotion recognition between our method (Personalized Emotion Recognition Model) and the baseline (General Emotion Recognition Model) across 20 participants. Our method, the personalized emotion recognition consistently yields lower MAE for the emotion estimation task.}
  \label{fig:personcompare}
\end{figure}
% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=0.7\linewidth]{Figs_v2/comparison_personspecific_0trail_v2.pdf}
%   \caption{Comparison of Mean Absolute Error (MAE) for emotion recognition between the baseline General Emotion Recognition Model and our Personalized Emotion Recognition Model across five participants (P1-P5) not present in the training data. Our method, the personalized approach consistently yields lower MAE for the emotion estimation task.}
%   \label{fig:personspecific}
% \end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[width=0.5\linewidth]{Figs_v2/fewshot.pdf}
  \caption{Emotion Estimation Error Reduction as the Number of Target Person's Traces Increases. The plot shows that the more traces from the target person are used, the better performance the model can reach with smaller errors.}
  \label{fig:fewshot}
\end{figure}


% \subsection{Performance of Trial Level Emotion Estimation v.s. Step Level Emotion Estimation}




==> Sections/not_used/05Discussion.tex <==
\section{Discussion}
\label{sec:discussion}
EmotionVibe can be combined with existing smart home devices to enhance human-device interactions. By inferring the users' emotional states through their footstep-induced floor vibrations, the system can modify the home's lighting, temperature, and even entertainment options, such as music and television recommendations accordingly to provide a more comfortable, supportive, and adaptive living environment. In addition, EmotionVibe can detect anomalies in emotional behavior that are often symptoms of mental health issues. Healthcare providers can intervene more effectively, offering timely support or modifying treatment regimens to better match the patient’s emotional and psychological state with people's emotional information.

In the future, we aim to extend EmotionVibe to real-world application scenarios to recognize mixed emotions, adapt to more diverse structural environments, and take various types of human activities into account:

\textbf{Expanding to Include Mixed Emotions:}
Human emotions are often mixed, with individuals experiencing multiple emotions simultaneously~\cite{larsen2014case,williams2002can,larsen2011further}. Mixed emotions can result in subtle and nuanced variations in gait or other behaviors that are difficult to categorize into singular emotional states. Future iterations of emotion recognition systems could explore techniques such as dynamic pattern recognition to discern and interpret these mixed emotional states.

\textbf{Expanding to Diverse Structures:}
In the future, we aim to adapt EmotionVibe to accommodate wider complex real-world environments with various structure types. It is important to improve the system's robustness and extend its applicability to various architectural structures, considering the unique acoustics and vibrations of different building materials such as wood, concrete, and steel. The structure materials can significantly influence the patterns of vibration signals used in emotion recognition. Developing a structure-invariant system can broaden its practical use in real-world environments.

\textbf{Expanding to Detect Various Activities:}
Emotions are reflected in a variety of daily activities, including working, gaming, and typing. Each type of activity corresponds to a unique behavioral pattern and physical interaction with the structure. Future research will explore EmotionVibe's capabilities to detect emotions from the structural vibrations induced by various activities. 

\textbf{Expanding to Natural Context:}
While our experiment offers a promising perspective on emotion recognition from footstep-induced floor vibrations, currently it relies upon data collected in a highly controlled lab setting. For instance, it is a well-studied experimental technique to elicitate emotions using music~\cite{warrenburg2020choosing}. 
It is important to replicate our findings within a more ecologically valid paradigm, where participants' natural emotional fluctuations are monitored using sensors installed in their homes.
